ACO-tagger: A Novel Method for Part-of-Speech Tagging using Ant Colony Optimization

Swarm Intelligence algorithms have gained significant attention in recent years as a means of solving complex and non-deterministic problems. These algorithms are inspired by the collective behavior of natural creatures, and they simulate this behavior to develop intelligent agents for computational tasks. One such algorithm is Ant Colony Optimization (ACO), which is inspired by the foraging behavior of ants and their pheromone laying mechanism. ACO is used for solving difficult problems that are discrete and combinatorial in nature. Part-of-Speech (POS) tagging is a fundamental task in natural language processing that aims to assign a part-of-speech role to each word in a sentence. In this research paper, proposed a high-performance POS-tagging method based on ACO called ACO-tagger. This method achieved a high accuracy rate of 96.867%, outperforming several state-of-the-art methods. The proposed method is fast and efficient, making it a viable option for practical applications.

==> refrences.tex <==
\begin{thebibliography}{1}
\bibitem{1}Jurafsky, D. \& Martin, J. Speech and Language Processing: An Introduction to Natural Language Processing, Computational Linguistics, and Speech Recognition.
\bibitem{2}Christopher, D. \& Hinrich, S. Foundations of statistical natural language processing. (the MIT press,1999)
\bibitem{3}Clark, S. \& Curran, J. Parsing the WSJ using CCG and log-linear models. {\em Proceedings Of The 42nd Annual Meeting Of The Association For Computational Linguistics (ACL-04)}. pp. 103-110 (2004)
\bibitem{4}Socha, K. \& Dorigo, M. Ant colony optimization for continuous domains. {\em European Journal Of Operational Research}. \textbf{185}, 1155-1173 (2008)
\bibitem{5}Dorigo, M. \& Gambardella, L. Ant colony system: a cooperative learning approach to the traveling salesman problem. {\em IEEE Transactions On Evolutionary Computation}. \textbf{1}, 53-66 (1997)
\bibitem{6}Dorigo, M., Maniezzo, V. \& Colorni, A. Ant system: optimization by a colony of cooperating agents. {\em IEEE Transactions On Systems, Man, And Cybernetics, Part B (Cybernetics)}. \textbf{26}, 29-41 (1996)
\bibitem{7}Schoonderwoerd, R., Holland, O. \& Bruten, J. Ant-like agents for load balancing in telecommunications networks. {\em Proceedings Of The First International Conference On Autonomous Agents}. pp. 209-216 (1997)
\bibitem{8}Dorigo, M. The Any System Optimization by a colony of cooperating agents. {\em IEEE Trans. System, Man & Cybernetics-Part B}. \textbf{26}, 1-13 (1996)
\bibitem{9}Deneubourg, J., Aron, S., Goss, S. \& Pasteels, J. The self-organizing exploratory pattern of the argentine ant. {\em Journal Of Insect Behavior}. \textbf{3} pp. 159-168 (1990)
\bibitem{10}Rabiner, L. A tutorial on hidden Markov models and selected applications in speech recognition. {\em Proceedings Of The IEEE}. \textbf{77}, 257-286 (1989)
\bibitem{11}Karbasian, H. \& Rashidi, P. PBT: PERSIAN PART OF SPEECH BRILL TAGGER. {\em IADIS Conference}. pp. 348-352 (2008)
\bibitem{12}Gharahbagh, A., Hajihashemi, V. \& Others A Persian part of speech tagging system using the long short-term memory neural network. {\em 2020 6th Iranian Conference On Signal Processing And Intelligent Systems (ICSPIS)}. pp. 1-6 (2020)
\bibitem{13}Hosseini Pozveh, Z., Monadjemi, A. \& Ahmadi, A. Persian texts part of speech tagging using artificial neural networks. {\em Journal Of Computing And Security}. \textbf{3}, 233-241 (2016)
\bibitem{14}Okhovvat, M. \& Bidgoli, B. A hidden Markov model for Persian part-of-speech tagging. {\em Procedia Computer Science}. \textbf{3} pp. 977-981 (2011)
\bibitem{15}Azimizadeh, A., Arab, M. \& Quchani, S. Persian part of speech tagger based on Hidden Markov Model. {\em 9th JADT}. (2008)
\bibitem{16}Besharati, S., Veisi, H., Darzi, A. \& Saravani, S. A hybrid statistical and deep learning based technique for Persian part of speech tagging. {\em Iran Journal Of Computer Science}. \textbf{4} pp. 35-43 (2021)
\bibitem{17}Bokaei, M., Sameti, H., Bahrani, M. \& Babaali, B. Segmental HMM-based part-of-speech tagger. {\em 2010 International Conference On Audio, Language And Image Processing}. pp. 52-56 (2010)
\bibitem{18}Church, K. A stochastic parts program and noun phrase parser for unrestricted text. {\em International Conference On Acoustics, Speech, And Signal Processing,}. pp. 695-698 (1989)
\bibitem{19}Bijankhan, M., Sheykhzadegan, J., Bahrani, M. \& Ghayoomi, M. Lessons from building a Persian written corpus: Peykare. {\em Language Resources And Evaluation}. \textbf{45} pp. 143-164 (2011)
\bibitem{20}Watanabe, O. \& Zeugmann, T. Stochastic Algorithms: Foundations and Applications: 5th International Symposium, SAGA 2009 Sapporo, Japan, October 26-28, 2009 Proceedings. (Springer Science & Business Media,2009)
\bibitem{21}Karaboga, D. \& Basturk, B. Artificial bee colony (ABC) optimization algorithm for solving constrained optimization problems. {\em Foundations Of Fuzzy Logic And Soft Computing: 12th International Fuzzy Systems Association World Congress, IFSA 2007, Cancun, Mexico, June 18-21, 2007. Proceedings 12}. pp. 789-798 (2007)
\end{thebibliography}

